Tracing The Start and End of Cosmic Reionization -- Exploring The Role of Ionizing Sources as drivers

This thesis investigates the Epoch of Cosmic Reionization (EoR), a key period in the early Universe when the first luminous sources formed and their radiation transformed the intergalactic medium (IGM) from neutral to ionized. Understanding this process reveals how the first stars and galaxies formed, influenced their surroundings, and shaped large-scale structures. The work traces both hydrogen and helium reionization by identifying the sources that produced ionizing radiation and examining how this radiation affected the thermal and ionization history of the IGM. Using the SPICE cosmological radiation-hydrodynamics simulations, the first part analyzes the ultraviolet luminosity function (UVLF) of high-redshift galaxies. It shows that different supernova feedback models drive distinct UVLF variability across mass and redshift, potentially alleviating the bright-galaxy tension seen by JWST. The second part explores how spectra from ionizing sources i.e. single and binary stars, X-ray binaries, emission from the interstellar medium, and active galactic nuclei impact the timing, topology, and thermal history of hydrogen reionization and the Lyman-alpha forest. At lower redshifts, radiative-transfer simulations reveal how helium reionization driven by quasars progressed and how the timing and temperature of the IGM relate to quasar luminosity functions and He II Ly-alpha observations. Finally, predictions for the 3.5 cm hyperfine transition of singly ionized helium-3 offer a novel probe of the post-reionization IGM. Together, these studies combine galaxy formation, radiative processes, and IGM evolution to provide a coherent picture of cosmic reionization and its observable signatures.

==> chapter/kap_03.tex <==

\chapter{The Influence of Ionizing Sources on Intergalactic Medium Properties}
\label{chap:chapter3}

\begin{flushright}
\begin{minipage}{0.5\textwidth}
\raggedleft
\textbf{\textit{``If I could wish for a thing, I would make neutrinos itchy for my enemies."}}\\[1ex]
\noindent\rule{0.5\textwidth}{0.4pt}\\[-0.2ex]
Géza Csörnyei
\end{minipage}
\end{flushright}

\begin{flushright}
\begin{minipage}{0.7\textwidth}
\raggedleft
\textbf{\textit{``Everything flows, no one can step into the same river twice, because everything flows and nothing stays."}}\\[1ex]
\noindent\rule{0.5\textwidth}{0.4pt}\\[-0.2ex]
Silvia Elizabeth Almada Monter
\end{minipage}
\end{flushright}



%\section{Overview}

\textit{This work has been submitted for publication in the Monthly Notices of the Royal Astronomical Society \citep{Basu2025b}.}

\hspace{1cm}

The growth of primordial density fluctuations from gravitational instabilities gave rise to the formation of the first stars and galaxies, which started to emit  photons with enough energy to ionize the surrounding intergalactic medium IGM and initiate the last global phase transition of the Universe, namely the Epoch of Reionization (EoR; \citealt{Loeb2001}). Observations of high-$z$ QSO absorption spectra \citep{Gunn1965,Fan2003,Fan2006,McGreer2015,bosman2018,Davies2018,Bosman2022}, Lyman-$\alpha$ emitters (LAEs; \citealt{Pentericci2014,Tilvi2014,Barros2017,Mason2018,Jung2022,Tang2023,Tang2024,nakane2024,napolitano2024,saxena2024,chen2024,ning2024}), information of the IGM thermal properties from QSO spectra \citep{Bolton2012,Raskutti2012,Gaikwad2020}, and of the Thompson scattering optical depth from the Cosmic Microwave Background (CMB; \citealt{Komatsu2011,planck2016,Pagano2020})
indicate that reionization is an extended process largely complete by $z= 5.5$, although patches of neutral hydrogen are found also at lower redshift \citep{kulkarni2019,nasir2020}. 

This abundance of observations is accompanied by an increasingly sophisticated modeling of the reionization process employing a variety of approaches, ranging from semi-analytic and semi-numeric models \citep{zhou2013,mesinger2007,santos2010,choudhury2018,hutter2021,choudhury2022}, to full radiation hydrodynamic simulations \citep{Baek2010,ocvirk2016,ockvirk2020, gnedin2014,finlator2018,Rosdahl2018,Trebitsch2021,kannan2022,garaldi2022,bhagwat2024}.
Although in most literature galaxies are thought to be the main drivers of reionization  \citep[e.g.][]{BeckerBolton2013,bouwens2015,robertson2015,Madau2017,dayal2020,hassan2018,Marius2020,eide2020b,kannan2022}, it is still unclear which are the properties of those contributing the most (e.g. small vs. massive galaxies; \citealt{Naidu2020,Naidu2021,Matthee2022}). Additionally, the recent detection of a larger than expected number density of faint quasars at intermediate (i.e. $z=4$; \citealt{Giallongo2015,Giallongo2019,Boutsia2018}) and high (i.e. $z>6$;  \citealt{Weigel2015,McGreer2018,Parsha2018,Akiyama2018,harikane2023,maiolinoa2023,Maiolino2023,Goulding2023,Larson2023,Juodzbalis2023,greene2023}) redshift, has renewed the interest in quasars as possible strong contributors to the ionization budget \citep{grazian2024,madau2024}.

Whatever the main source of ionizing photons is, the physical properties of the IGM in terms of ionization and thermal state are influenced by a variety of sources, including the above mentioned stars and quasars, but also X-ray binaries (XRBs; \citealt{mirabel2011,fragos2013,fragosa2013,madaufragos2017,sazonov2017}), Bremsstrahlung emission from shock heated interstellar medium (ISM; \citealt{Chevalier1985,suchkov1994,strickland2000}), low energy cosmic rays \citep{nath1993,sazonov2015,leite2017,owen2019,bera2023,yokoyama2023,gessey2023,carvalho2024}, self-annihilation or decay of dark matter \citep{liu2016,cang2023} and plasma beam instabilities in TeV blazars \citep{chang2012,puchwein2012,lamberts2022}. 

As discussed for example in \citealt{Marius2018} and \citealt{Marius2020} (but see also, \citealt{Baek2010,venkatesan2011,Grissom2014,enrico2019}), the more energetic sources are responsible for the partially ionized and warm gas found outside of the regions fully ionized by stars. Additionally, they can also increase the IGM temperature in comparison to the one obtained in star driven reionization scenarios. 
Their impact on studies of the 21cm signal from neutral hydrogen at high-$z$ has been widely recognized and investigated \citep{ross2017,ross2019,qingbo2020,qingbo2021,qingbo2022,kamran2022,cook2024,noble2024}.
Such high-energy sources may also impact the Ly$\alpha$ forest by broadening thermal widths and thereby increasing the transmission flux. 

Traditionally, emissivity models in reionization studies focus on the cumulative contribution of ionizing photons from evolving stellar populations, often incorporating time-dependent source formation histories to estimate the global photon budget. However, in this study, I adopt a different approach. While I still utilize an emissivity-based framework, my focus is not on the integrated luminosity evolution over time, but rather on how variations in the spectral energy distribution SED of the sources influence Ly$\alpha$ forest observables. By isolating the impact of SED shape, assuming a fixed emissivity model, I aim to determine whether different assumptions about the source spectra can significantly alter interpretations of the Ly$\alpha$ forest. The chapter is organized as follows: Section~\ref{methodology} outlines the simulations, Section~\ref{results} presents my findings, and Section~\ref{discussion} concludes with a broader interpretation of the results.



\begin{figure*}   
\centering
    \includegraphics[width=50mm]{figures/emissivity.pdf} 
    \includegraphics[width=50mm]{figures/SED_models.pdf}  
    \includegraphics[width=50mm]{figures/gammahi.pdf}
    \caption{ \textit{Left Panel:}Redshift evolution of the total ionizing photon rate adopted in this study (solid line) with a compilation of observational constraints \citep{becker2021,gaikwad2023,davies2024}. \textit{Middle Panel:} averaged spectral energy distribution $\bar{S}(\nu,z)$ for: single stars (\texttt{SS}, red curve); a combination of single stars, ISM and XRBs (\texttt{SS+ISM+XRBs}, blue curve); a combinination of binary stars, ISM and XRBs (\texttt{BS+ISM+XRBs}, green curve); a black-body spectrum with $T$=50000 K (\texttt{BB}); a power-law spectrum with a slope of -3 (\texttt{SOFT-PL}); a power-law spectrum with a slope of -1.8 (\texttt{AGN-PL}). The vertical gray lines indicate the ionization thresholds for neutral hydrogen (13.6 eV), neutral helium (24.6 eV) and singly ionized helium (54.4 eV).  \textit{Right Panel:} The resulting H~{\sc i} photoionization rate for all six models with a compilation of observational constraints \citep{Calverley2011,wyithe2011,daloisio2018,Davies2018, davies2024}.}
    \label{fig:siminput}
\end{figure*}


\section{Methodology}
\label{methodology}
Here, I describe how I have post-processed the outputs of a hydrodynamical simulation (Section \ref{hydrosim}) with the multi-frequency radiative transfer (RT) code \texttt{CRASH} (Section \ref{crash}) to obtain a suite of simulations of reionization (Section \ref{section:2.3}).

\subsection{The cosmological hydrodynamic simulation}
\label{hydrosim}

To obtain the gas and source distribution and properties, I have used outputs at redshift 5.16 to 15 from a Sherwood-type hydrodynamical simulation  performed in a comoving cubic box of size 20 $h^{-1}$ Mpc \citep{bolton2016}, with the parallel Tree-PM smoothed particle hydrodynamics (SPH) code \texttt{p-GADGET-3},   which is an updated version of \texttt{GADGET-2} \citep{Volker2001,gadget2}. The box contains $2\times1024^{3}$ gas and dark matter particles, each of mass $m\rm{_{gas}}=9.97 \times 10^{6} M_{\odot}$ and  $m\rm{_{DM}}=5.37 \times 10^{7} M_{\odot}$, respectively. Haloes are identified using the friends-of-friends algorithm with a linking length of $0.2$ times the mean inter-particle separation. The gravitational softening length for the simulation is set to 1/30th of the mean linear interparticle spacing, and star formation is incorporated using a simple and computationally efficient prescription which converts all gas particles with overdensity $\Delta > 10^{3}$ and temperature $T<10^{5} \rm{K}$ into collisionless stars \citep{Viel2004,viel2013}. Note that because of this simple treatment, the simulation does not self-consistently model star formation and feedback, but is perfectly appropriate to investigate IGM properties \citep{keating2016,kulkarni2016,mallik2024}. The Sherwood model adopts a Planck 2013 consistent cosmology  \citep{planck2013} with $\rm{\Omega_{m}=0.308}$, $\rm{\Omega_{\Lambda}=0.692}$, $\rm{\Omega_{b}=0.0482}$, $\rm{\sigma_{8}=0.829}$, $\rm{\mathit{n}_{s}=0.963}$, $h=0.678$, where the symbols have their usual meaning.
Throughout the chapter, the gas is assumed to be of primordial composition with a hydrogen and helium number fraction of 0.92 and 0.08, respectively, and no metals.

\subsection{The radiative transfer code \texttt{CRASH}}
\label{crash}
The radiative transfer of ionizing photons through the IGM is implemented by post-processing the outputs of the hydrodynamic simulation using the 3D non-equilibrium and multi-frequency code \texttt{CRASH}  \citep[e.g.][]{ciardi2001,maselli2003,maselli2009,graziani2013,hariharan2017,glatzle2019,glatzle2022}. The code evaluates self-consistently the ionization states of hydrogen and helium, as well as the evolution of gas temperature. \texttt{CRASH} employs a Monte Carlo-based ray tracing approach, where the propagation of ionizing radiation is represented by multi-frequency photon packets that dynamically trace the spatial and temporal distribution of radiation within the simulation volume. The version of \texttt{CRASH} employed here has a comprehensive treatment of UV and soft X-ray photons, including X-ray ionization, heating, and secondary electron interactions \citep{graziani2018}. For an in-depth understanding of \texttt{CRASH}, I encourage readers to refer to the foundational papers.

\subsection{The radiative transfer simulation of reionization}
\label{section:2.3}

To post-process the simulation outputs with \texttt{CRASH}, I have gridded the gas density and temperature extracted from the snapshots onto $N_{\rm grid}^{3}$ cells.
More specifically, the RT is performed with $N_{\rm grid}=128$ (corresponding to a spatial resolution of 156 $h^{-1}\,\mathrm{ckpc}$) in the range $z=15-8$, while at $z<8$ the resolution is increased to $N_{\rm grid}=256$ (corresponding to 78 $h^{-1}\,\mathrm{ckpc}$) to ensure a better description of the Ly$\alpha$ forest related statistics. The gridded properties of the gas are obtained by assigning the particle data to a regular grid using the SPH kernel \citep{monaghan1992}, while the corresponding grid for the halo masses and positions is obtained by using the cloud-in-cell and friends-of-friends algorithms \citep{hockney1988,springel2001}. If more than one halo end up in the same cell, their masses are combined. 
To reduce the large number of sources present in the simulation box and thus the computational time, I have adopted the source clustering technique developed by \citet{Marius2020} with a luminosity limit of $0.1$ and maximum radius of $\sqrt{2}\times 2.01$ (see the original paper for more details). Every ionizing source emits $10^{4}$ photon packets which are lost once they exit the simulation box, i.e. no periodic boundary condition has been used. 

For each output $i$ at $z_i$ of the hydrodynamical simulation, the RT is followed for a time $\rm{\mathit{t}_{H}(\mathit{z}_{i+1}) - \mathit{t}_{H}(\mathit{z}_{i})}$, where $\rm{\mathit{t}_{H}(\mathit{z}_{i})}$ is the Hubble time corresponding to $z_{i}$. 
In order to account for the expansion of the Universe between the $i$-th and $(i+1)$-th snapshots, the gas number density is evolved as $n(\mathbf{x},z) = n(\mathbf{x}, z_{i})(1 + z)^{3}/(1 + z_{i})^{3}$, where $\mathbf{x} \equiv (x_{c}, y_{c}, z_{c})$ are the coordinates of each cell $c$. To avoid accounting twice for the UV background (which is already included in the hydrodynamic simulations), at $z\leq9$ all cells with $\rm{\mathit{T}<10^5 K}$ are assigned a temperature $\rm{\mathit{T}_{i+1}=\mathit{T}_{i}(1+\mathit{z}_{i+1}^{2})/(1+\mathit{z}_{i}^{2}}$), i.e. only the effect of the adiabatic cooling since the previous snapshot is taken into account in the evolution of the temperature, while the photoheating due to the UVB is discarded.  For the cells with $\rm{\mathit{T}\geq10^{5} K}$, the value of the temperature is not changed to take into account the heating from shocks, which is not captured by the RT (see also \citealt{maselli2003,whalen2008,Iliev2009,Cain2024} for additional details). 
The ionization fractions are initialized to their expected residual values from the recombination epoch i.e.  $x_{\rm HII}=10^{-4}$ and  $x_{\rm HeII}=x_{\rm HeIII}=0$.

The source emissivity is evaluated according to the prescription introduced by \citet{Ciardi2012}, namely, I have assumed a total comoving hydrogen ionizing emissivity at each redshift, $\epsilon\rm{_{tot}(\mathit{z}_i)}$, and distributed it in terms of rate of ionizing photons (${\dot{N}_{\text{ion}}}$) among all the halos  proportionally to their mass. I display my adopted redshift evolution of ${\dot{N}_{\text{ion}}}$ in the left panel of Figure \ref{fig:siminput}. This approach assures by design that the  emissivity is broadly consistent with $z= 5-6$ observations \citep{becker2021,gaikwad2023,davies2024}, however there is discrepancy between the observations. 
Additionally, it does not require any assumption on the escape fraction of ionizing photons, which is a very uncertain quantity (\citealt{vanzella2016,vanzella2018,matthee2018,naidu2018,steidel2018,fletcher2019}; for a review see \citealt{wood2000,Pratika2018}). Differently from \citet{Ciardi2012}, though, rather than having a purely linear relation between the ionizing emissivity and the halo mass, I have incorporated a Gaussian noise with mean $\mu=0$ and standard deviation $\sigma=0.01$ in the log-log scale, conserving the total ionizing emissivity (as done in \citealt{enrico2019,Basu2024}).

The spectral energy distribution (SED) of the sources has been derived following 
\citealt{Marius2018,Marius2020,qingbo2022}, which include the contribution from single (SS) and binary (BS) stars, XRBs and thermal Bremsstrahlung from supernova-heated ISM. While I refer the reader to the original papers for more details, here I note 
that stars dominate the total SED budget at energy $\rm{\mathit{h}_p \nu \leq 60}$ eV, while the ISM contribution is dominant above that into hard UV and the soft X-rays (i.e.in the range $\rm{\mathit{h}_p \nu \in [60,500]}$ eV),  and the XRBs start to contribute  at $\rm{\mathit{h}_p \nu > 500}$ eV (see Figure 2 in \citealt{Marius2018} and Figure 1 in \citealt{qingbo2022} for a visual inspection). 
For all RT simulations, the spectra of ionizing sources extend to a maximum frequency of $\rm{\sim 2 \ keV}$ and are discretized into 82 frequency bins, with  bins more densely spaced around the ionization thresolds of hydrogen (13.6 eV) and helium (24.6 eV and 54.4 eV). I run three reference simulations: one with ionizing sources consisting solely of single stars (\texttt{``SS"}), another adding also the contribution from the ISM and XRBs (\texttt{``SS+ISM+XRBs"}), and a third that includes binary stars along with the ISM and XRBs (\texttt{``BS+ISM+XRBs"}). For comparison, I also perform three additional simulations using simplified SED prescriptions commonly adopted in the literature. These include a blackbody spectrum with $T$ = 50,000 K (\texttt{``BB"}), a galaxy-like power-law SED with a slope of -3 (\texttt{``SOFT-PL"}), and an AGN-type power-law SED with a slope of -1.8 (\texttt{``AGN-PL"}). For simplicity, following \citealt{Marius2018,Marius2020}, I adopt the globally averaged SEDs (averaging over the spectral shapes for all sources) for the first three simulations. For the last three simulations, I assume a constant model for all sources. The resulting SEDs for all six simulations are shown in the middle panel of Figure \ref{fig:siminput}. 



\begin{figure*}
    \includegraphics[scale=0.355]{figures/xHII_maps_z6_allmodels.pdf}     
    \includegraphics[scale=0.355]{figures/xHeII_maps_z6_allmodels.pdf}      
    \includegraphics[scale=0.355]{figures/xHeIII_maps_z6_allmodels.pdf}   
    \includegraphics[scale=0.355]{figures/temp_maps_z6_allmodels.pdf}   
    \caption{From top to bottom, slice maps of the H~{\sc ii}, He~{\sc ii}, He~{\sc iii} fractions  and IGM temperature at $z= 6$ for different combinations of SED models: single stars  ({\tt SS}, first column);  single stars, ISM and XRBs ({\tt SS+ISM+XRBs}, second); binary stars, ISM and XRBs ({\tt BS+ISM+XRBs}, third); blackbody ({\tt BB}, fourth); galaxy power law ({\tt SOFT-PL}, fifth) and AGN power law ({\tt AGN-PL}, sixth). The lower sets of rows show the difference with respect to the simulations with single stars only. The maps are $20 h^{-1} \rm{cMpc}$ wide and $78 h^{-1} \rm{ckpc}$ thick.}
    \label{fig:slice_map}
\end{figure*}

%\begin{figure}
%    \includegraphics[width=\columnwidth]{figures/xHII_slicemap_z6_allb_all.pdf}  
%    \caption{Difference map of the H~{\sc ii} fraction comparing the simulations {\tt BS+ISM+XRBs} (with binary stars) to {\tt SS+ISM+XRBs} (without binary stars) at $z= 6$, illustrating the impact of including binary stars in the simulation. The map spans a width of $20 h^{-1} \mathrm{cMpc}$ and a thickness of $78 h^{-1} \mathrm{ckpc}$.}
%    \label{fig:slice_map_diff_allb_all}
%\end{figure}

 

\section{Results}
\label{results}


The central question I seek to explore is: \textit{what is the impact of SED models on the properties of the IGM as revealed by the Ly$\alpha$ forest?} To address this, I will first examine the resulting photoionization rate and the qualitative differences introduced by different SEDs of sources, then delve into the resulting reionization and thermal histories. Finally, I will analyze their influence on the observable features associated with the Ly$\alpha$ forest.

\subsection{H~{\sc i} photoionization rate}
\label{photoionizationrate}
In the right most panel of Figure \ref{fig:siminput}, I present the H~{\sc i} photoionization rate ($\rm{\mathit{\Gamma}_{HI}}$) extracted from my simulations at $z \lesssim 8$, where a higher spatial resolution for the RT calculations is achieved (as discussed in Section \ref{section:2.3}). The results are shown for all simulations, alongside observational constraints from \citealt{Calverley2011,wyithe2011,daloisio2018,Davies2018,davies2024}, and estimates from \citealt{puchwein2018} including contributions from both galaxies and AGNs. All simulations follow a similar overall trend, with $\rm{\mathit{\Gamma}_{HI}}$ increasing by approximately an order of magnitude from $z = 8$ to $z = 5$. At $z = 6$, the evolution of $\rm{\mathit{\Gamma}_{HI}}$ slows down and eventually flattens, marking the phase when the majority of the simulation volume becomes ionized.

When comparing the different models to the \texttt{SS} reference simulation, I observe that despite the general trend being similar, differences emerge. Notably, the \texttt{SOFT-PL} model consistently yields the largest $\rm{\mathit{\Gamma}_{HI}}$ value, higher by a factor of $\sim 1.15$ compared to \texttt{SS}. This difference arises primarily due to a slightly lower number of photons in the H~{\sc i} ionization regime for \texttt{SOFT-PL}, as inferred from the SED models in Figure \ref{fig:siminput}. Meanwhile, models with more consistent SEDs in this regime—\texttt{BB}, \texttt{SS+ISM+XRBs}, and \texttt{BS+ISM+XRBs}—exhibit similar trends, with \texttt{BB} producing the highest $\rm{\Gamma_{HI}}$.
The behavior of the \texttt{AGN-PL} model is particularly interesting, as at the highest redshifts it exhibits the lowest $\rm{\Gamma_{HI}}$ value, which primarily happens because much of the volume is already ionized, leading to a decrease in the photoionization rate. However, it becomes higher than all the other models (except for \texttt{SOFT-PL}) at $z = 6$, reaching a peak before declining again, indicating the completion of the reionization process. In the following sections, I conduct a detailed analysis of IGM ionization and heating by  comparing the impact of different source SEDs on the Ly$\alpha$ forest.

\subsection{Qualitative Overview of IGM properties}
\label{slice_compare}

For a qualitative discussion of the results, Figure \ref{fig:slice_map} presents maps of the ionization and thermal state of the IGM at $z = 6$ for all simulations, together with maps showing the difference relative to \texttt{SS}.

In the \texttt{SS} model, the gas is mostly either fully ionized and hot ($x_{\rm HII} \approx x_{\rm HeII} \approx 1$, $T_{\rm IGM} \gtrsim 10^4$ K) or nearly neutral and cold ($x_{\rm HII} \approx x_{\rm HeII} \lesssim 10^{-4}$, $T_{\rm IGM} \sim 10$ K). While ionized regions are mainly shaped by radiation from single stars, there are slight traces of partial ionization and heating, mostly due to resolution effects, as large scale numerical simulations can not resolve the ionization front correctly for short mean free paths. In contrast, the \texttt{SS+ISM+XRBs} model introduces extra heating and partial ionization outside of the fully ionized regions, due to the high-energy photons emitted by the ISM and XRBs, raising the gas temperature by few hundred degrees. This is evident in the difference maps of H~{\sc ii}, He~{\sc ii}, and $\rm{\mathit{T}_{IGM}}$, where red pixels highlight regions with increased ionization and heating. He~{\sc ii} behaves similarly to H~{\sc ii}, with the exception that within fully ionized regions He~{\sc ii} is partially converted into He~{\sc iii}, as it is clearly visible from both maps and difference maps. The impact of He~{\sc iii} is also seen as an increment in the temperature of the ionized regions. I also note that the noise-like pattern in the $\rm{\mathit{T}_{IGM}}$ difference maps within fully ionized regions results from Monte Carlo noise, as obtaining exactly the same temperature between simulations with different ionizing sources is statistically unlikely. However, this is not the case for the ionization fraction once a cell is fully ionized. 

The inclusion of binary stars in the \texttt{BS+ISM+XRBs} simulation introduces further differences in the ionization and thermal structure of the IGM. Since binary stars produce a larger number of H~{\sc i} and He~{\sc i} ionizing photons, H~{\sc ii} regions are more extended compared to the \texttt{SS} model. This is visible in the difference maps, where darker red areas appear around fully ionized regions. A similar feature is also seen in the temperature maps.
Notably, the \texttt{BS+ISM+XRBs} model results in a slightly lower He~{\sc iii} fraction than \texttt{SS+ISM+XRBs} because a significant fraction of ionizing photons is consumed in expanding the ionized bubbles, while the total ionizing photon budget per time step remains fixed. 
\begin{figure}
\centering
\includegraphics[width=100mm]{figures/xHI_evolution_all_models.pdf}   
    \caption{{\it Top panel:} Redshift evolution of the volume averaged $\mathit{x}\rm{_{HI}}$ for all SED models: \texttt{SS} (red curve), \texttt{SS+ISM+XRBs} (blue), \texttt{BS+ISM+XRBs} (green), \texttt{BB} (orange), \texttt{SOFT-PL} (yellow) and \texttt{AGN-PL} (purple). The symbols denote a compilation of observational constraints from the literature \citep{Bosman2022,fan_2006,Davies2018,Mason2018,McGreer2018,greig2017,greig2019,hoag2019,yang2020,umeda2024,durovcicova2024,nakane2024,spina2024,zhu2024, Mason2025}. {\it Bottom panel:} Fractional difference with respect to the \texttt{SS} simulation.}
    \label{fig:XHIevol}
\end{figure}

%The difference maps in Figure \ref{fig:slice_map_diff_allb_all} emphasize these effects, showing dark red patches surrounding ionized regions, indicating their expansion due to binary stars. For the same reason, the amount of partial ionization is slightly lower compared to \texttt{SS+ISM+XRBs} model.

Compared to the \texttt{SS} model, the \texttt{BB} model shows slightly smaller partially ionized regions around ionized bubbles, though this is mainly due to resolution effects. However, the extent of fully ionized regions in the \texttt{BB} model is slightly smaller, as seen from the dark blue patches around ionized areas in the difference maps of $x_{\rm HII}$ and $x_{\rm HeII}$. The amount of doubly ionized helium is higher in \texttt{BB}, since this model produces more photons at and slightly beyond the He~{\sc ii} ionization energy compared to the \texttt{SS} model. The temperature difference maps reveal regions with $\Delta T_{\rm IGM} \sim -100$ K, indicating slightly lower photoheating in the \texttt{BB} model. This is primarily because the total number of photons emitted is the same, so if the \texttt{BB} model has more photons with energy $ \geq 54.4$ eV, which ionise He~{\sc II} with little heating, it will have less photons at energy $< 54.4$ eV, which provide more heating. However, the presence of more extended helium double ionization regions introduces some additional heating.

In the \texttt{SOFT-PL} model the extent of fully ionized regions is even smaller, indicating a delayed reionization process. This aligns with the higher overall H~{\sc i} photoionization rate seen in Figure \ref{fig:siminput}. The \texttt{SOFT-PL} model also has a higher fraction of gas partially ionized by the higher energy tail of the SED, with many cells reaching $x_{\rm HII} \sim 10^{-2}$. The difference maps reveal filamentary structures with positive $\Delta x_{\rm HII}$, representing regions that were ionized earlier in the \texttt{SS} model but later cooled and recombined due to their high density. Additionally, the He~{\sc iii} fraction reaches values as high as $x_{\rm HeIII} \sim 10^{-1}$. The temperature maps further reflect this, showing increased heating in the partially ionized regions. Inside ionized bubbles, especially in dense areas, there is a combined effect of delayed reionization and additional helium double ionization heating, with the former being the dominant factor.

In the \texttt{AGN-PL} model, all the effects discussed above are even more pronounced. The higher number of high-energy photons leads to stronger partial ionization of H~{\sc i} and He~{\sc i}, with many cells reaching $x_{\rm HII}$ and $x_{\rm HeII} \sim 10^{-1}$. These energetic photons also drive more helium double ionization, creating large regions of fully ionized helium. As a result, the overall temperature is significantly higher, and the temperature difference maps appear mostly red, reflecting widespread heating across the slice. Apart from that, the extent of the fully ionized regions of H~{\sc ii} and He~{\sc ii} is slightly smaller than in  the \texttt{SS} model. 

While these differences highlight the qualitative impact of various SED model assumptions, in the following sections I will focus on a more quantitative analysis. 

\subsection{Reionization history}
\label{sec:reion}
To discuss the overall effect induced by different SED models, in Figure \ref{fig:XHIevol} I display the redshift evolution of the volume averaged H~{\sc i} fraction for all simulations, together with the fractional difference with respect to  \texttt{SS}, and a compilation of observational results \citep{fan_2006, greig2017, greig2019, Davies2018, Mason2018, McGreer2018, hoag2019, yang2020, Bosman2022, umeda2024, durovcicova2024, nakane2024, spina2024, zhu2024, Mason2025}. By design, all simulations are consistent with observational constraints at $z \lesssim 5.5$, where my primary focus lies. The curves are able to reproduce most data points also at higher redshift, where though there is less consistency among different observations.  

As discussed earlier, including binary stars or more energetic sources leads to increased ionization, resulting in a lower H~{\sc i} fraction. The largest differences occur at $z = 5.6$, where the \texttt{SS+ISM+XRBs} and \texttt{BS+ISM+XRBs} models show deviations of about 7.5$\%$ and 10$\%$, respectively. In contrast, the \texttt{BB} model has a higher H~{\sc i} fraction up to $z = 5.6$, indicating a slightly delayed reionization (of about $\Delta z \sim 0.05$) compared to the \texttt{SS} model. This delay is even stronger in the \texttt{SOFT-PL} and \texttt{AGN-PL} models, which maintain higher H~{\sc i} fractions over a similar redshift range. The \texttt{SOFT-PL} model shows the largest deviation, exceeding a fractional difference of 150$\%$ at $z=5.6$, while the deviation for \texttt{AGN-PL} model reaches about 100$\%$. This is mainly due to smaller extent of fully ionized regions in the \texttt{SOFT-PL} and \texttt{AGN-PL} models, as discussed in Section \ref{slice_compare}, causing a slightly slower reionization process. 
As reionization continues and $\langle x_{\rm HI} \rangle$ drops below $10^{-4}$, the differences between models decrease and eventually disappear. However, during the final phases of reionization, the \texttt{SOFT-PL} and \texttt{AGN-PL} models predict a  Universe more ionized than in the \texttt{SS} model, with deviations of $\sim$15$\%$ and 30$\%$, respectively.

\begin{figure}
\centering
\includegraphics[width=100mm]{figures/T0_evolution_all_models.pdf}   
    \caption{{\it Top panel:} Redshift evolution of the IGM temperature at mean density ($\mathit{T}\rm{_{0}}$) for \texttt{SS} (red curve), \texttt{SS+ISM+XRBs} (blue), \texttt{BS+ISM+XRBs} (green), \texttt{BB} (orange), \texttt{SOFT-PL} (yellow) and \texttt{AGN-PL} (purple). The symbols denote a compilation of observational constraints from the literature \citep{Bolton2012,boera2019,Gaikwad2020}. {\it Bottom panel:} Fractional difference with respect to the \texttt{SS} simulation.}
    \label{fig:tempevol}
\end{figure}

\subsection{Thermal history}
\label{thermal_history}
The ionization of hydrogen and helium injects energy into the IGM through photo-heating, raising its temperature, and consequently affecting the dynamics of gas, its cooling rate, and its accretion onto galaxies. In Figure \ref{fig:tempevol} I show the redshift evolution of the IGM temperature at mean density, calculated by selecting all the cells in the simulation volume with gas density within 1\% of the mean density.  
As expected, with the exception of \texttt{AGN-PL}, $ T_{0} $ rises with decreasing redshift, reaching a peak at $ z= 6 $ when about 99\% of the simulation volume is ionized. Subsequently, the rate of heat injection from photo-heating diminishes, leading to a plateau followed by a gradual decline, which is much shallower, though, than the one  suggested by a compilation of observational data \citep{Bolton2012,boera2019,Gaikwad2020}. 
The shallower evolution observed is primarily due to additional heating associated to the increasing number of cells experiencing hydrodynamical feedback effects (with cells having IGM temperature $> 10^{5}$ K), which remain challenging to disentangle or accurately correct for while post processing with the RT code. This behavior has already been discussed in the context of helium reionization by \citealt{basu2024}. 
Interestingly, the \texttt{SOFT-PL} and \texttt{AGN-PL} models deviate from this trend, showing no significant decline in $T_0$. While the \texttt{SOFT-PL} model exhibits a brief saturation at $z = 6$, the temperature continues to rise at lower redshifts, primarily due to the effects of helium double ionization. A similar trend is evident in the \texttt{AGN-PL} model, though with a significantly higher amplitude, consistently exceeding the temperatures of other models by more than 7500 K due to the abundant energetic photons populating this SED. This highlights the sustained influence of AGNs on the thermal evolution of the IGM, but also it is not consistent with the observational constraints, differently from the evolution of the H~{\sc i} fraction.


\begin{figure}
\centering
    \includegraphics[width=120mm]{figures/LOS_z5_all_models.pdf}
    %\includegraphics[width=58mm]{LOS_z5_5.pdf}
    %\includegraphics[width=87mm]{LOS_z5.pdf}
    \caption{IGM properties along a reference line of sight at \textit{z} = 5 for \texttt{SS} (red curve), \texttt{SS+ISM+XRBs} (blue), \texttt{BS+ISM+XRBs} (green), \texttt{BB} (orange), \texttt{SOFT-PL} (yellow) and \texttt{AGN-PL} (purple). From top to bottom the panels refer to the H~{\sc i} fraction, IGM temperature, Ly$\alpha$ optical depth, and normalized transmission flux. 
    }
    \label{fig:los}
\end{figure}

Both \texttt{SS+ISM+XRBs} and \texttt{BS+ISM+XRBs} exhibit temperatures higher than \texttt{SS} due to additional heating from more energetic photons, with binary stars contributing even more significantly. The maximum temperature difference reaches approximately $5\%$ at $z = 8$, but gradually decreases to about $1\%$ at lower redshifts, as reionization progresses.  
%By $z = 5$, the \texttt{SS+ISM+XRBs} and \texttt{BS+ISM+XRBs} simulations have effectively converged. This is primarily because the presence of binary stars accelerates ionization and photo-heating, allowing sufficient time for cooling to occur. Meanwhile, in the \texttt{SS+ISM+XRBs} simulation, $T_0$ continues to rise until it eventually aligns with the temperature in the binary star simulation.  
The \texttt{BB} model consistently shows lower temperatures, with a nearly constant deviation of $\sim 4\%$ for $z \lesssim 6$. Differently, \texttt{SOFT-PL}  initially produces temperatures lower than the \texttt{SS} model, reaching a maximum negative deviation of $\sim 10\%$ at $z = 8$. However, below $z = 6$, this deviation gradually decreases and eventually turns positive, reaching approximately $8\%$ at $z = 5$. 
As already mentioned, the \texttt{AGN-PL} model is characterized by larger values of $T_0$ at all redshifts, with deviations of $\sim 100\%$.


In the following I will investigate if the differences in IGM temperature and ionization state affect the Ly$\alpha$ forest properties.


\subsection{Ly$\alpha$ forest statistics}
\label{lyalpha_forest}
To investigate Ly$\alpha$ forest properties, I have generated synthetic spectra by extracting 16384 sightlines at each RT snapshot, each spanning the full box length parallel to the $z$-direction. For each pixel $i$ in a sightline I evaluate the normalized transmission flux $F(i) = \exp[-\tau(i)]$, where
\begin{equation}
    \tau(i) = \frac{c \sigma_{\alpha} \delta R}{\sqrt{\pi}} \sum_{j=1}^{N} \frac{n\mathrm{_{HI}}(j)}{b\mathrm{_{HI}}(j)} \ \tilde{V}(i,j)
\end{equation}
is the Ly$\alpha$ optical depth. Here $N$ is the number of pixels in a sightline, $\sigma_{\alpha}$ is the Ly$\alpha$ scattering cross-section, $c$ is the speed of light, $\delta R$ is the size of a pixel in proper distance units, $n_\mathrm{{HI}}(j)$ is the H~{\sc i} number density at the position of pixel $j$, $\mathrm{\mathit{b}_{HI}(\mathit{j}) = (2 \mathit{k}_{B} \mathit{T}_{IGM} / \mathit{m}_{H})^{1/2}}$, $\mathrm{\mathit{k}_{B}}$ is the Boltzmann constant, $\mathrm{\mathit{m}_{H}}$ is the hydrogen mass, and $\tilde{V}$ is the convoluted Voigt profile approximation provided by \citealt{tepper2006}. The latter depends on the IGM temperature and the peculiar velocity. Throughout this chapter, I ignore the contamination from other lines into the wavelength window of the Ly$\alpha$ forest, and notice that this is not expected to have any impact on my results \citep{hellsten1998,yang2022}.


\begin{figure}   
\centering
\includegraphics[width=100mm]{figures/taueff_evolution_all_models.pdf}
    \caption{{\it Top panel:} Redshift evolution of the Ly$\alpha$ effective optical depth for \texttt{SS} (red curve), \texttt{SS+ISM+XRBs} (blue), \texttt{BS+ISM+XRBs} (green), \texttt{BB} (orange), \texttt{SOFT-PL} (yellow) and \texttt{AGN-PL} (purple). The shaded regions indicate 95$\%$ confidence intervals. The symbols denote a compilation of observational constraints from the literature \citep{fan_2006,Becker2015,eilers2018,yang2020,bosman2018,Bosman2022}. {\it Bottom panel:} Fractional difference with respect to the \texttt{SS} simulation.}
    \label{fig:taueff_evol}
\end{figure}

\subsubsection{Individual lines of sight}
\label{los}

As a reference, in Figure \ref{fig:los} I display the neutral hydrogen fraction ($\rm{\mathit{x}_{HI}}$), the IGM temperature ($\rm{\mathit{T}_{IGM}}$), the Ly$\alpha$ optical depth ($\rm{\tau}$), and the Ly$\alpha$ transmitted flux ($F$) along a single line of sight (LOS) at $z=5$. For clarity, I omit the pixel index when referring to the values of these physical quantities.

The abundance of H~{\sc i} remains remarkably consistent across all simulations, with only slight variations. Notably, a marginally lower value is observed in the {\tt AGN-PL} model, as illustrated also in Figure~\ref{fig:XHIevol}. 
The ionized regions are characterized by an IGM temperature $T_{\rm IGM} \sim 10^4$~K, with  {\tt AGN-PL} exhibiting the highest value of $\sim 10^{4.4}$~K, as discussed in previous sections. In all models the highest temperatures are reached in regions which have been recently ionized. 
The behavior observed in the H~{\sc i} fraction is directly reflected in the corresponding Ly$\alpha$ optical depth ($\tau$), which has typical values below 5 in regions of higher ionization. It is in these areas that I also observe a larger transmission of Ly$\alpha$ photons.

When comparing different SED models, the {\tt AGN-PL} consistently exhibits the highest transmission, suggesting that its additional heating affects the width and shape of transmission features.
Instead, the other models do not show substantial variations in the transmitted flux, as the differences in optical depth introduce only subtle fluctuations, with the {\tt SOFT-PL} model exhibiting the smoothest transmission profile, primarily driven by the additional heating which slightly enhances the transmission by reducing small-scale variations in optical depth.  
The {\tt SS+ISM+XRBs} and {\tt BS+ISM+XRBs} models follow a similar trend, but with slightly reduced smoothness and marginally lower transmission. In contrast, the {\tt SS} model, which lacks additional heating contributions, displays more suppressed transmission, with a sharper and more irregular flux profile.
Finally, the {\tt BB} model exhibits the lowest Ly$\alpha$ transmission among all cases, indicating a more neutral IGM with reduced transparency to Ly$\alpha$ photons. 

While the characteristics discussed above are common to the majority of lines of sight, to provide a more quantitative comparison, in the next sections I calculate quantities which more accurately capture the statistical behavior of the Ly$\alpha$ forest. 

\subsubsection{Evolution of the effective optical depth}

The first statistical quantity I discuss is the Ly$\alpha$ effective optical depth ($\tau_{\rm eff}$), a widely used characterization of the Ly$\alpha$ forest. To calculate this, I combine multiple synthetic spectra to obtain a length of 50$\rm{\mathit{h}^{-1} cMpc}$ (typically adopted in observational papers, e.g. \citealt{Bosman2022}), resulting in over $\sim 5500$ sightlines at each redshift. The effective optical depth for each los is then computed as:
\begin{equation}
\tau_{\rm{eff}} = - \ln (\langle F \rangle),
\label{columndensity}
\end{equation}
where $\langle F \rangle$ is the mean transmitted flux of all the pixels in each new sightline. Figure \ref{fig:taueff_evol} displays the redshift evolution of the median $\tau_{\rm eff}$, along with the central $95 \%$ of the data, as well as a compilation of observational constraints from \citealt{fan_2006,Becker2015,eilers2018,bosman2018,yang2020,Bosman2022}. It is important to note that the input emissivity in the \texttt{SS} simulation is calibrated to match the observational estimates of $\langle \rm F \rangle$ at $z \lesssim 5.5$ \citep{Becker2015,eilers2018,bosman2018,Bosman2022}. As the emissivity is same in all simulations, this ensures that the reference model is consistent with empirical data, while allowing me to examine deviations in the other models. All simulations produce a very similar behavior, with $\tau_{\rm eff}$ decreasing with the progress of reionization, and slightly flattening at $z\lesssim6$. It is also interesting to see that all models are consistent with the majority of observational data within the scatter.

As can be better appreciated in the bottom panel of the figure, for $z \gtrsim 6$, the differences between models, with the exception of {\tt AGN-PL} and {\tt SOFT-PL}, are modest, with a maximum deviation from the {\tt SS} model of $\sim 1\%$, which becomes $<0.5\%$ at $z\sim5$ for {\tt SS+ISM+XRBs} and {\tt BS+ISM+XRBs}. This suggests that the SEDs of BS, ISM and XRBs do not significantly alter the effective optical depth, while the deviation remains at the 1\% level for a black-body spectrum. 
On the other hand, both {\tt SOFT-PL} and {\tt AGN-PL} at $z=5$ produce an effective optical depth which is $\sim 10\%$ lower than the {\tt SS} one, highlighting the impact of the larger abundance of more energetic photons, which produce a higher transmission of Ly$\alpha$ photons in comparison to the other models. The higher effective optical depth for the {\tt AGN-PL} model at $z\gtrsim6.5$ is mostly due to higher impacts of H~{\sc i} although having much higher temperature compared to other models.

\subsubsection{Distributions of Ly$\alpha$ Transmission Flux}

\begin{figure}
\centering
    \includegraphics[width=105mm]{figures/F_dist_z5_6_all_models.pdf}
    \caption{{\it Top panels:} Distribution of the Ly$\alpha$ transmission flux for \texttt{SS} (red curve), \texttt{SS+ISM+XRBs} (blue), \texttt{BS+ISM+XRBs} (green), \texttt{BB} (orange), \texttt{SOFT-PL} (yellow) and \texttt{AGN-PL} (purple) at  $z=5$ (\textit{left panel}) and 6 (\textit{right}). {\it Bottom panels:} Fractional difference with respect to  the \texttt{SS} simulation.}
    \label{fig:Fpdf}
\end{figure}

To provide a more statistical perspective on the variations in transmitted flux across different models, in Figure~\ref{fig:Fpdf} I present its distribution, computed over the entire sample of sightlines at $z=6$ and $z=5$. The overall pattern is similar for all models, with more pixels having low transmission (i.e. more absorption) due to the patchy nature of the reionization process.  
As reionization proceeds and the IGM becomes more transparent to Ly$\alpha$ photons, the fraction of pixels with $F \gtrsim 0.5$ increases, while low-transmission pixels become less common. By $z=5$, when reionization is complete, the flux distribution is almost flat for $0.2 \lesssim F \lesssim 0.8$.

When comparing the various models, I find that, except for {\tt SOFT-PL} and {\tt AGN-PL}, the differences in flux distribution relative to {\tt SS} are generally small, typically below 2\%, meaning that variations in the sources SED have only a minor effect on transmission. The largest differences appear at the highest transmission levels ($F > 0.9$), where the {\tt SS+ISM+XRBs} and {\tt BS+ISM+XRBs} models show a $\sim$5\% increase in the number of high-transmission pixels\footnote{Note that the results at $z=6$ are less robust due to the fewer pixels with higher Ly$\alpha$ transmission at this redshift.}.
In contrast, both the {\tt SOFT-PL} and {\tt AGN-PL} models show much larger deviations (as high as 100\% and 1000\%, respectively) at both redshifts, with a significantly higher fraction of pixels with $F \gtrsim 0.2$. Also for these models the deviation increases at higher transmission levels. These results highlight the strong impact of ionization and heating driven by sources with a power-law SED, such as AGNs, which render the IGM more transparent compared to models without such sources.







\subsubsection{1-D Flux Power Spectra}
\label{lya_ps}

\begin{figure}   
\centering
    \includegraphics[width=95mm]{figures/PS_all_models.pdf}
    \caption{{\it Top panels:} 1-D dimensionless Ly$\alpha$ forest transmission flux power spectra at $z=5$ (\textit{left panel}) and 5.6 (\textit{right}) for \texttt{SS} (red curve), \texttt{SS+ISM+XRBs} (blue), \texttt{BS+ISM+XRBs} (green), \texttt{BB} (orange), \texttt{SOFT-PL} (yellow) and \texttt{AGN-PL} (purple). The symbols denote a compilation of observational constraints from the literature \citep{boera2019}.
    {\it Bottom panel:} Fractional difference with respect to  the \texttt{SS} simulation along with the uncertainties of the observational constraints.}
   \label{fig:ps_w_scaling}
\end{figure}

I calculate The 1-D power spectrum (PS) of Ly$\alpha$ transmission flux using all sightlines from my simulation, and plot it in Figure~\ref{fig:ps_w_scaling} at $z=5$ and $z=5.6$. The latter redshift is chosen because it is when the largest differences  in $\langle \rm{\mathit{x}_{HI} \rangle}$ emerge, and at the same time there are enough regions of high transmission to render my exploration of their fluctuations more statistically significant.  The overall shape of the power spectra is similar at both redshifts, increasing from $k \sim 10^{-0.5} \ \mathrm{s \ km^{-1}}$ to $k \sim 10^{-1.6} \ \mathrm{s \ km^{-1}}$, which marks the typical scale of fluctuations in the Ly$\alpha$ forest, and then decreasing at larger scales. However, the power at $z=5$ is lower than at $z=5.6$ because by then the IGM is mostly ionized, making the Ly$\alpha$ transmission more uniform. 
The saturation in power at the highest $k$-values comes mostly from the limitation of the thermal broadening kernel which affects small-scale accuracy. 
By comparing my results to observational data from \citealt{boera2019} at $z=5$, that all models match them well, with the exception of \texttt{AGN-PL} at $k \gtrsim 10^{-1.2}$. 

At $z=5.6$, I observe that the models with contribution from more energetic sources, \texttt{SS+ISM+XRBs} and \texttt{BS+ISM+XRBs}, show only a slight deviation from the \texttt{SS} model, with a small $0.5\%$ increase in the flux power spectrum at $k \sim 10^{-1.6} \, \mathrm{s \, km^{-1}}$. This enhancement is localized, with differences disappearing at both the smallest and largest scales. Within $10^{-1.3} \text{ s km}^{-1} \lesssim k \lesssim 10^{-0.8} \text{ s km}^{-1}$, the power spectrum slightly decreases due to the effect of thermal Doppler broadening associated with photoheating, which leads to broader absorption features and reduces fluctuations. This effect is more pronounced in the \texttt{BS+ISM+XRBs} model, as it produces a slightly higher IGM temperature. Other SED models show larger deviations. The \texttt{BB} and \texttt{SOFT-PL} models have a similar behaviour, which results in a power spectrum higher (lower) than the {\tt SS} one at small (large) spatial scales, although the differences are still within a few percent (and up to 8\% for \texttt{SOFT-PL}). This results from differences in the H~{\sc i} distribution due to inhomogeneous ionization on large scales, and from a combined effect of ionization, recombination in dense regions, and photoheating on small scales. 
The \texttt{AGN-PL} model stands out as at low $k$ it has about $10\%$ higher fluctuations than \texttt{SS} due to differences in H~{\sc i} distribution, while at higher $k$ the power drops before peaking again at a $10\%$ deviation, driven by additional heating from helium double ionization. As the IGM becomes more homogeneous by $z=5$, fluctuations diminish, leaving residual deviations mainly influenced by the presence of He~{\sc ii}, which slightly modifies the UV background, along with thermal Doppler broadening from increased temperatures. By this stage, most models show only a $2\%$ deviation compared to the \texttt{SS} model, except for \texttt{AGN-PL}, which remains at $10\%$.

Such small differences remain within the observational uncertainties reported by \citealt{boera2019} for the Ly$\alpha$ 1-D flux power spectrum at $z=5$, with the exception of the extreme \texttt{AGN-PL} model. While current observations make it difficult to isolate the impact of different SEDs on the flux power spectrum, surveys with next-generation facilities like the Extremely Large Telescope (\texttt{E-ELT}) and upgraded Dark Energy Spectroscopic Instrument (\texttt{DESI}) could reduce the error bars to $1\%$–$2\%$, enabling a more precise assessment of how to distinguish the contribution from sources with different SED models. Achieving this level of accuracy would be a major step forward in understanding the bias in the interpretations of observations of Ly$\alpha$ forest assuming a certain SED model.


\subsubsection{Galaxy-IGM connection}
\label{gal-igm}

\begin{figure*}
\centering
\includegraphics[width=50mm]{figures/excess_transmission_z_6_0.pdf}
\includegraphics[width=50mm]{figures/excess_transmission_z_6_5.pdf}
\includegraphics[width=50mm]{figures/excess_transmission_z_7.pdf}
    \caption{{\it Top panels:} Excess Ly$\alpha$ forest transmission at $z=6$ (left panel), 6.5 (middle) and 7 (right) for \texttt{SS} (red curve), \texttt{SS+ISM+XRBs} (blue), \texttt{BS+ISM+XRBs} (green), \texttt{BB} (orange), \texttt{SOFT-PL} (yellow) and \texttt{AGN-PL} (purple). The symbols denote a compilation of observational constraints from the literature \citep{meyer2019,meyer2020,kashino2023}.
    {\it Bottom panel:} Fractional difference with respect to  \texttt{SS} simulation along with the uncertainties of the observational constraints for the sample of haloes with $\rm{\mathit{M}_{halo} \geq 10^{10} M_{\odot}}$ (upper part) and the full sample of haloes (lower part).}
    \label{fig:excess_transmission}
\end{figure*}

To investigate more in detail the local effect of different SED models, 
I examine how the transmissivity ($T$) varies with distance $r$ from nearby galaxies. This approach, first proposed by \citealt{kakiichi2018} and subsequently adopted also by \citealt{meyer2019, meyer2020, kashino2023}, provides a complementary way to probe the relation between sources and their surrounding IGM. 
A key finding from these works is that the Ly$\alpha$ transmitted flux shows a broad peak at intermediate distances from ionizing sources, which can be interpreted as due to a proximity effect, suggesting that galaxies enhance ionization in their immediate surroundings, leading to increased Ly$\alpha$ transmissivity. While observational studies have made significant progress in this area \citep{koki2025}, theoretical investigations remain limited, with the exception of \citealt{garaldi2022,garaldi2024}, who examined this phenomenon using high-resolution radiation-hydrodynamics simulations, and  \citealt{conaboy2025},  who employed models of patchy reionisation.

Following the efforts made by \citealt{garaldi2022} to create a synthetic version of observations, in Figure \ref{fig:excess_transmission} I present the excess IGM transmissivity relative to its average across all $r$, expressed as $ \langle T(r) \rangle / \bar{T} - 1 $, at $ z = 6 $, 6.5, and 7. However, comparing my simulations with observations is challenging due to the different methods used to collect data. For instance, \citealt{meyer2019} identified galaxies based on C~{\sc iv} absorption along quasar sightlines, while \citealt{meyer2020} used Ly$\alpha$ emitters (LAEs) and Lyman-break galaxies (LBGs). More recently, \citealt{kashino2023} employed [O~{\sc iii}] emitters for galaxy identification. To facilitate a meaningful comparison, I show excess transmission for both - haloes with $ \rm{M_{halo} \geq 10^{10} M_{\odot}} $ and the full sample of haloes. my simulations reveal an excess transmissivity at smaller distances ($ r \leq 10 $ ${\rm cMpc}$), with a higher amplitude at earlier times, which declines by $ z = 6 $. This trend suggests that ionized regions were more compact and concentrated around galaxies at higher redshifts. The excess at $z=6$ transmission is more pronounced for the most massive haloes compared to the full sample, likely due to their stronger ionizing radiation output. Interestingly, while my results show excess transmission at shorter distances than \citealt{meyer2019, meyer2020}, they align more closely with the findings of \citealt{kashino2023}. At larger distances ($ r \geq 20 $ ${\rm cMpc}$), my results show better agreement with observations, although \citealt{kashino2023} reports a sharp decline after $ r \geq 12 $ ${\rm cMpc}$. At $z=6.5$, my simulations overpredict the excess Ly$\alpha$ transmission till $r=10 {\rm \ cMpc}$ compared to observational constraints from \citealt{meyer2019}, however beyond that, my results align much better with them. However, looking at the nature of the observational datapoints, excess transmission region in \citealt{meyer2019} lies slightly at the higher distance. As redshift increases from $ z = 6 $ to $ z = 7 $, I observe that the amplitude of excess transmission increases and shifts to larger distances. This behavior arises due to three key factors: (i) lower overdensities at earlier times, which limit the suppression of Ly$\alpha$ flux near galaxies due to weaker hydrogen recombination; (ii) smaller ionized bubbles at higher redshifts, which restrict the distance at which flux is enhanced; and (iii) a rapid decline in the average transmissivity $ \bar{T} $ at earlier times, while highly ionized regions continue to produce localized transmission spikes. These factors collectively shape the evolution of Ly$\alpha$ transmissivity and its dependence on galaxy proximity over cosmic time. Towards the greater distances (i.e. $r \geq 20 {\rm \ cMpc}$), all models converge as excess transmission approaches zero, since local transmission aligns with the global mean.

In the bottom panels of Figure \ref{fig:excess_transmission}, I present the fractional difference in excess transmission relative to the \texttt{SS} model, along with observational uncertainties from \citealt{meyer2019, meyer2020, kashino2023}. At all redshifts, deviations are noisier for halos with $ \rm{M_{halo} \geq 10^{10} M_{\odot}} $ compared to the full sample. At $ z = 6 $, in the closest regions around sources ($ r \lesssim 9 $ ${\rm cMpc}$), the \texttt{AGN-PL}, \texttt{SOFT-PL}, and \texttt{BB} models exhibit higher excess transmission, reaching a maximum deviation of $ \sim 1000 \% $ gradually increasing towards higher end of the distance. This is slightly lower for the full sample. In contrast, the \texttt{BS+ISM+XRBs} model shows the lowest excess transmission, while the \texttt{SS+ISM+XRBs} model transitions from negative deviations at $ r \lesssim 6.5 $ ${\rm cMpc}$ to positive ones at larger distances. Observational uncertainties generally exceed the fractional deviations, but at certain distances, deviations in some models surpass observational constraints. At $ z = 6.5 $, the transition to positive excess transmission shifts to $ r \lesssim 4 $ ${\rm cMpc}$, though limited data restrict direct comparisons. By $ z = 7 $, this region contracts further to $ r \leq 2 $ ${\rm cMpc}$. In the range where positive excess transmission occurs, the \texttt{AGN-PL}, \texttt{SOFT-PL}, and \texttt{BB} models show the highest deviations, forming a peak before declining at the outer edge, a trend most noticeable at $ z = 6.5 $ and $ z = 7 $, while excess transmission diminishes at $ z = 6 $. In these regions, the \texttt{BS+ISM+XRBs} and \texttt{SS+ISM+XRBs} models exhibit negative deviations, meaning their excess transmission is about 10\% lower than that of the \texttt{SS} model. Observational uncertainties are comparable to deviations in most cases, but at some distances in both $ z = 6.5 $ and $ z = 6 $, the \texttt{AGN-PL}, \texttt{SOFT-PL}, and \texttt{BB} models exceed them, suggesting they may be distinguishable within observational limits. Even at the largest distance, while some instances show deviations exceeding observational uncertainties, most remain within error bars, highlighting the distinct behaviors of different ionizing source models and their potential for observational testing.


\section{Conclusion and Discussion}
\label{discussion}
This work investigates the influence of SED modelling considering non-stellar ionizing sources, including X-ray binaries, Bremsstrahlung emission from shock heated ISM, and binary stars, on the IGM during the epoch of reionization. I perform a comparative study of these SED models with standard assumptions like a power law or blackbody spectrum. Using tailored radiative transfer simulations post-processed on hydrodynamical outputs from the Sherwood suite, I explored the impact of these SED models on Ly$\alpha$ forest observables. By comparing simulations with distinct SEDs, including those dominated by single stars, binary stars, and additional high-energy sources, I assessed their contributions to the ionization and thermal histories of the IGM and their impact on observable properties such as the Ly$\alpha$ flux and its power spectrum.

The main results can be summirized as follows:
\begin{itemize}
    \item The morphology of ionized regions in the IGM varies significantly depending on the spectral energy distribution SED of ionizing sources. In the reference model with only single stars (SS), the IGM appears as a patchwork of fully ionized hot regions and cold, neutral surroundings. When additional energetic components such as ISM and XRBs are included, partially ionized and heated regions appear beyond the ionization fronts. Models including binary stars (BS) show even more extended H~{\sc ii} regions, due to a higher photon production rate, though this expansion slightly reduces the He~{\sc iii} content since more photons are used in ionizing hydrogen. The \texttt{AGN-PL} model stands out by producing widespread heating and partial ionization across the full volume, resulting in a more uniformly ionized and thermally elevated IGM. 
    
    \item All SED models show a general increase in the hydrogen photoionization rate ($\rm{\mathit{\Gamma}_{HI}}$) from $z = 8$ to $z = 5$, flattening at lower redshifts as reionization concludes. Among the models, \texttt{SOFT-PL} yields the highest $\rm{\mathit{\Gamma}_{HI}}$ values due to its spectrum being more concentrated around the hydrogen ionization threshold. The blackbody (\texttt{BB}) model also shows elevated rates. In contrast, the \texttt{AGN-PL} model exhibits a more complex evolution—starting with low $\rm{\mathit{\Gamma}_{HI}}$ at high redshift, overtaking other models at $z \approx 6$, before declining again, indicating a peak in ionizing influence around the end of reionization.

    \item The evolution of the volume-averaged neutral hydrogen fraction is sensitive to the source SED. Models that include ISM, XRBs, or binary stars ionize the IGM more efficiently, leading to a faster drop in $\langle x_{\rm HI} \rangle$ compared to the \texttt{SS} model. On the other hand, the \texttt{BB}, \texttt{SOFT-PL}, and \texttt{AGN-PL} models show delayed reionization, with \texttt{SOFT-PL} exhibiting up to 150$\%$ higher $\langle x_{\rm HI} \rangle$ than \texttt{SS} at $z \approx 5.6$. Interestingly, by the end of reionization ($z \lesssim 5.5$), the \texttt{AGN-PL} and \texttt{SOFT-PL} models predict a Universe more than the \texttt{SS} model due to their sustained photon production in harder spectral regimes.
    
    \item The IGM temperature at mean density increases as reionization progresses, peaking at $z \approx 6$ for most models. The \texttt{SS+ISM+XRBs} and \texttt{BS+ISM+XRBs} configurations show modest increases in temperature compared to \texttt{SS}, driven by additional photoheating. The \texttt{BB} model results in slightly cooler temperatures, due to fewer photons in the heating-optimal range. The \texttt{SOFT-PL} model initially has a temperature lower than \texttt{SS}, but eventually it becomes larger due to heating associated to helium double ionization. The \texttt{AGN-PL} model consistently produces much higher temperatures —exceeding \texttt{SS} by more than 7500 K at $z = 5$ due to the large fraction of high-energy photons in its SED, although this scenario is inconsistent with observational constraints.

    \item When inspecting individual lines of sight at $z = 5$, most models show similar hydrogen fractions and temperature distributions, with minor differences in Ly$\alpha$ optical depth and transmitted flux. The \texttt{AGN-PL} model shows the highest temperatures and the greatest transmitted flux, owing to stronger heating and broader absorption features. In contrast, the \texttt{BB} model shows lower flux due to its relatively neutral and cooler IGM. Other models fall between these extremes, with smoother profiles observed in the \texttt{SOFT-PL} case.
    
    \item The flux PDF evolves with redshift as the IGM becomes more ionized. At $z = 5$, all models show a broader distribution of high-transmission pixels. The \texttt{BB} and \texttt{SS} models produce the most absorption (lowest flux), while \texttt{AGN-PL} and \texttt{SOFT-PL} shift the distribution toward higher fluxes, especially in the range $F > 0.2$. These models show deviations exceeding 100$\%$ in the fraction of high-transmission pixels relative to SS, reflecting their enhanced ionization and heating capabilities.
    
    \item The 1D power spectrum of Ly$\alpha$ transmission flux exhibits differences across SED models, particularly at $z = 5.6$ when reionization is still ongoing. Most models show only minor deviations ($\lesssim$2$\%$) from the \texttt{SS} model, with changes localized to intermediate scales due to thermal broadening. \texttt{AGN-PL} shows the most significant differences, up to 10$\%$ higher power on large scales due to spatial ionization variations and 10$\%$ lower power on small scales from extreme heating. These signatures, while subtle, could be observable with future high-precision spectroscopic surveys.

    \item All models replicate the general decline of the Ly$\alpha$ effective optical depth ($\tau_{\rm eff}$) with redshift, consistent with existing observational constraints. Differences among models are subtle, generally within 1$\%$ for  $z \lesssim$ 6. However, the \texttt{AGN-PL} and \texttt{SOFT-PL} models yield $\tau_{\rm eff}$ values up to 10$\%$ lower than the \texttt{SS}  reference model at $z = 5$ due to their higher ionization and heating efficiency. At higher redshifts ($z \gtrsim$ 6.5), the \texttt{AGN-PL} model shows slightly higher $\tau_{\rm eff}$ due to delayed reionization in high-density regions.

    \item By analyzing Ly$\alpha$ transmission as a function of distance from galaxies, I observe enhanced transmissivity (proximity effect) within $\sim$10 ${\rm \ cMpc}$ of massive halos. This effect is strongest at earlier times ($z =$ 7), when ionized regions are smaller and the IGM is more neutral. Hard-spectrum sources like \texttt{AGN-PL} and \texttt{SOFT-PL} produce the strongest proximity effects, while stellar models, particularly BS+ISM+XRBs, show more modest enhancements. These results align with recent observational studies and suggest that proximity zone statistics could distinguish between different source populations in the reionization era.
\end{itemize}

This study underscores the critical role of SED models impacting the observational interpretations of Ly$\alpha$ forest. By integrating diverse ionizing sources, the simulations provide a more complete picture of the IGM's evolution, advancing my understanding of the interplay between astrophysical sources and cosmological processes. These findings hold significant implications for the astrophysical community. As future observational campaigns, such as those utilizing the Extremely Large Telescope (\texttt{E-ELT}) or advanced iterations of \texttt{DESI}, achieve unprecedented precision in measuring the Ly$\alpha$ flux power spectrum, it will become possible to disentangle the relative contributions of various source populations. Incorporating such insights into models will refine constraints on reionization and the thermal history of the Universe. Continued exploration of high-energy sources, particularly their impact on small-scale IGM structures, represents a promising avenue for future research.

==> chapter/kap_05.tex <==
\chapter{Probing Helium reionization through the $^{3}\mathrm{He}^{+}$ transition line}
\label{chap:chapter5}

\begin{flushright}
\begin{minipage}{0.7\textwidth}
\raggedleft
\textbf{\textit{``Everyone has one, but don't be one to each other."}}\\[1ex]
\noindent\rule{0.5\textwidth}{0.4pt}\\[-0.2ex]
Joanne Tan
\end{minipage}
\end{flushright}

\begin{flushright}
\begin{minipage}{0.7\textwidth}
\raggedleft
\textbf{\textit{``Where we go from there is a choice I leave to you."}}\\[1ex]
\noindent\rule{0.5\textwidth}{0.4pt}\\[-0.2ex]
Akash Vani (\textit{inspired from `The Matrix'})
\end{minipage}
\end{flushright}



\textit{This work has been submitted for publication in the Monthly Notices of the Royal Astronomical Society \citep{Basu2025c}.}

\hspace{1cm}


At redshift $z \approx 1100$, hydrogen recombined as the Universe expanded and cooled sufficiently to allow electrons to bind with protons. At earlier times ($z \approx 6000$), helium experienced its first recombination (He~{\sc iii} $\to$ He~{\sc ii}), i.e. the one pertaining its inner electron, which is bound with an energy of 54.4 eV \citep{Switzer2008b}. As the Universe continued to cool, singly ionized helium (He~{\sc ii}) recombined into neutral helium (He~{\sc i}) at $z\approx 1800$ \citep{Switzer2008a}. 
With time, the neutral atoms formed during these recombination epochs were gradually reionized by photons emitted from various emerging astrophysical sources.
As the first ionization potential of helium is similar to the one of hydrogen, He~{\sc i} is expected to be ionized into He~{\sc ii} at the same time of hydrogen, i.e. by $z \sim 5.5$ \citep{Fan2006,Becker2015,bosman2018,Bosman2022}. However, the reionization of singly ionized helium (He~{\sc ii} $\to$ He~{\sc iii}) occurs at a later time, requiring the energetic photons emitted by quasars \citep{Compostella2013,upton2016,daloisio2017,Mitra2018,Garaldi2019,Basu2024}. 

Following hydrogen recombination, the IGM comprised approximately $24\%$ helium by number, predominantly in the form of $^4\mathrm{He}$, with a much smaller abundance of $^3\mathrm{He}$—about one part in $10^5$ relative to $^4\mathrm{He}$ \citep{kneller2004}. The $^3\mathrm{He}$ isotope is particularly significant due to its nonzero magnetic dipole moment, which enables hyperfine splitting in the hydrogen-like $^3\mathrm{He}^+$ ion, resulting in a rest-frame transition at 8.67 GHz (3.5-cm), analogous to the well-known 21-cm line from neutral hydrogen \citep{field1959,madau1997,shaver1999,tozzi2000,furnaletto2006,ciardi2003,zaroubi2013,acharya2024}. While much of the effort to explore the high-redshift IGM has focused on the 21-cm line, the $^3\mathrm{He}^+$ hyperfine transition offers a unique window into key astrophysical processes in the early Universe \citep{furnaletto2006, bagla2009, McQuinn2009, takeuchi2014, vasiliev2019}. Since the evolution of \textsc{H ii} and He~{\sc ii} during the Epoch of Reionization (EoR) is primarily driven by stellar sources, the resulting signals at 21-cm and 3.5-cm are expected to be anti-correlated. Because of that, as proposed by \citealt{bagla2009}, beyond tracing the high-$z$ evolution of the helium component in the IGM, the 3.5-cm signal could also provide constraints independent from those of the 21-cm signal. Additionally, this line can help to constrain the properties of ionizing sources and serve as a powerful mean for detecting quasars \citep{khullar2020}. It also has a potential to probe large scale filamentary structures as discussed by \citealt{takeuchi2014}.

Although the abundance of He~{\sc ii} is lower than the one of \textsc{H ii}, the $^3\mathrm{He}^+$ hyperfine transition has several advantages over the 21-cm line: (i) the foreground contamination is smaller at higher rest-frame frequency , and (ii) its spontaneous decay rate is $\sim 680$ times larger, enhancing the signal strength. However, the detectability of this signal is limited by the sensitivity of most current telescopes. While there are several radio telescopes which are operating in this relevant frequency range, the Square Kilometre Array (\texttt{SKA}) (specifically in the Phase 2, using \texttt{SKA-mid}) is the most promising one to detect this signal. 

While \citealt{bagla2009} estimated the signal strength using semi-analytic methods, more detailed numerical simulations are necessary to capture the full complexity of He~{\sc ii} evolution, including spatial inhomogeneities, radiative transfer effects, and feedback mechanisms that semi-analytic models may not fully incorporate. \citealt{takeuchi2014} provided a precise estimation of the ionization state of $^3\mathrm{He}^+$ and studied the physical processes that influence its spin temperatures over a wide redshift range ($z \sim 0-8$). However, their work did not include radiative transfer effects, which are crucial for a more accurate representation of how ionizing radiation propagates through the IGM. 
The investigation by \citealt{khullar2020} addressed some of these limitations by using radiative transfer simulations (\citealt{Marius2020}) to explore the possibility of detecting the $^3\mathrm{He}^+$ signal, considering various ionizing sources, including stars, X-ray binaries, accreting black holes, and shock-heated gas in the interstellar medium. Additionally, they also studied a high-$z$ quasar to investigate its environment (see also, \citealt{koki2017}). However, a more detailed investigation at lower redshifts, where helium reionization is ongoing, is crucial for assessing the feasibility of detecting the 3.5 cm signal over a wider redshift range. Since the impact of quasars on reionization is redshift-dependent, focusing on this later stage provide new insights into how the evolving He~{\sc ii} ionizing radiation field influences the IGM.

Recent observational work has sought to constrain the prospects of helium hyperfine signal detection. \citealt{Trott2024} presented the first limits on the power spectrum  of the $^3\mathrm{He}^+$ hyperfine transition at $z = 3{-}4$ on spatial scales of 30 arcminutes, using 190 hours of archival interferometric data from the Australia Telescope Compact Array (ATCA). Although noise and residual radio frequency interference limited their sensitivity, the study demonstrated the feasibility of detecting the helium signal with current telescopes. It also emphasized the potential of next-generation instruments, such as \texttt{SKA}, which, with their higher sensitivity, could yield cosmologically relevant signals and offer deeper insights into helium reionization.

Here, I present a detailed study of helium reionization focussing on the lower redshift IGM ($z < 5$) with insights from simulated $^3\mathrm{He}^+$ hyperfine transition line utilising the latest cosmological simulations of helium reionization \citep[][hereafter AB24]{Basu2024}. I also perform a quantitative comparison between the simulated $^3\mathrm{He}^+$ signal and the first observational constraints from \citealt{Trott2024}. The simulation incorporates recent constraints on the Quasar Luminosity Function (QLF) and successfully reproduces the majority of helium reionization observations, including the He~{\sc ii} Lyman-$\alpha$ forest. Specifically, I introduce the simulation methodology in Section \ref{method}, present the results in Section \ref{results}, and conclude with a discussion in Section \ref{conclusion}. Throughout this work, I adopt a flat $\Lambda \rm{CDM}$ cosmology, consistent with \cite{Planck2016}, using the following parameters: $\Omega_{\rm m} = 0.3089$, $\Omega_{\Lambda} = 0.6911$, $\Omega_{\rm b} = 0.0486$, $h = 0.6774$, $\sigma_{8} = 0.8159$, and $n_{\rm s} = 0.9667$, where the symbols have their usual meanings.

\begin{figure*}
\centering
    \includegraphics[width=160mm]{figures/helium_deltatbmaps.pdf}
    \caption{Slice map of $^3\rm{He}^+$ differential brightness temperature across the simulation box at $z\approx4.18$, 3.28 and 2.90, from left to right.  The maps are 205$\rm{\mathit{h}^{-1} cMpc}$ wide and 400$\rm{\mathit{h}^{-1} ckpc}$ thick.}
    \label{deltatb_map}
\end{figure*}

\section{Methods}
\label{method}

\subsection{Simulation of helium reionization}

In the following, I briefly describe the simulation used to estimate the 3.5~cm signal, while I refer the reader to AB24 for more details. 

The radiative transfer (RT) simulation has been performed by post-processing the \texttt{TNG300} hydrodynamical simulation, which is part of the \texttt{Illustris TNG} project \citep{volker2018,naiman2018,marinacci2018,pillepich2018,nelson2018}. This simulation was performed using the \texttt{AREPO} code \citep{springel2010}, which solves the idealized magneto-hydrodynamical equations \citep{pakmor2011} governing the non-gravitational interactions of baryonic matter, as well as the gravitational interactions of all matter. \texttt{TNG300} employs the latest \texttt{TNG} galaxy formation model \citep{weinberger2017,pillepich2018}, with star formation implemented by converting gas cells into star particles above a density threshold of $\textit{n}\rm{_{H}} \sim 0.1 \ \rm{cm^{-3}}$, following the Kennicutt-Schmidt relation \citep{springel2003}. The simulation is run in a comoving box of length $L_\mathrm{box} = 205 \,h^{-1} \, \mathrm{cMpc}$, with (initially) $2 \times 2500^{3}$ gas and dark matter particles. The average gas particle mass is $\bar{m}\rm{_{gas}} = 7.44 \times 10^{6} \, M_{\odot}$, while the dark matter particle mass is fixed at $m\rm{_{DM}} = 3.98 \times 10^{7} \, M_{\odot}$. Haloes are identified on-the-fly using a friends-of-friends algorithm with a linking length of $0.2$ times the mean inter-particle separation.  I utilized 19 outputs covering the redshift range $5.53 \leq z \leq 2.32$.

The radiative transfer of ionizing photons through the IGM has been implemented with the \texttt{CRASH} code \citep[e.g.][]{ciardi2001,maselli2003,maselli2009,Maselli2005,partl2011}, which computes self-consistently the evolution of hydrogen and helium ionization states, as well as gas temperature. \texttt{CRASH} employs a Monte Carlo-based ray-tracing scheme, where ionizing radiation and its spatial and temporal variations are represented by multi-frequency photon packets propagating through the simulation volume. The latest version of \texttt{CRASH} includes UV and soft X-ray photons, accounting for X-ray ionization, heating, detailed secondary electron physics \citep{graziani2013,graziani2018}, and dust absorption \citep{glatzle2019,glatzle2022}. For more details, I refer the reader to the original \texttt{CRASH} papers. The RT is performed on grids of gas density and temperature extracted from \texttt{TNG300} snapshots and tracks radiation with energy $h_p \nu \in [54.4 \ \mathrm{eV}, 2 \ \mathrm{keV}]$, assuming fully ionized hydrogen (i.e. $x_{\rm HI} = 10^{-4}$) and fully singly ionized helium (i.e. $x_{\rm HeI} = 0$). 

As sources of ionizing radiation I consider quasars, which are assigned to halos in the simulation according to a modified abundance-matching approach (see AB24 for more details) to reproduce the QLF of \citealt{Shen2020}.
The quasar SED is the same adopted in \citealt{Marius2018} and \citealt{Marius2020}, which is obtained by averaging over 108,104 SEDs observed in the range $0.064 < z < 5.46$ \citep{Krawczyk2013} at $h_P \nu <200$~eV, while it follows a power law with index $-1$ at higher energies (see Section 2 of \citealt{Marius2018}). 

\subsection{The 3.5~cm signal}

The simulation described in the previous section provides the spatial and temporal distributions of the gas number density, $\rm{\mathit{n}_{gas}}$, and temperature, $\rm{\mathit{T}_{gas}}$, as well as of the fractions of H~{\sc ii}, He~{\sc ii}, and He~{\sc iii} (denoted as $\rm{\mathit{x}_{HII}}$, $\rm{\mathit{x}_{HeII}}$, and $\rm{\mathit{x}_{HeIII}}$, respectively). 
The brightness temperature associated with the hyperfine transition of $^{3}\mathrm{He}^{+}$, $\rm{\mathit{\delta T}_{b,^{3}He}}$, is evaluated in each cell of the simulated volume as (see eq.~61 of \citealt{furnaletto2006}):

\begin{align}
    \rm{\mathit{\delta T}_{b,^{3}He}} \approx & \ 0.5106 \ \rm{\mathit{x}_{HeII} \ (1+\delta) \ (1 - \frac{\mathit{T}_{CMB}}{\mathit{T}_{s}})}
    & \times \ \rm{(\frac{[^{3}He/H]}{10^{-5}}) \ (\frac{\Omega_{b}\mathit{h}^{2}}{0.0223}) \sqrt{\frac{\Omega_{m}}{0.24}} \ (1+\mathit{z})^{1/2} \ \mu K}, 
    \label{deltatb_formula}
\end{align}
where $\delta = (\mathit{n}_{\mathrm{gas}} - \bar{\mathit{n}}_{\mathrm{gas}})/\bar{\mathit{n}}_{\mathrm{gas}}$ is the gas overdensity, with $\bar{\mathit{n}}_{\mathrm{gas}}$  mean gas number density within the simulation box. $\mathit{T}_{\mathrm{CMB}} = 2.725(1+\mathit{z}) \, \mathrm{K}$ denotes the CMB temperature at redshift $z$, $\rm{\mathit{T}_{s}}$ is the spin temperature, and the relative abundance of $^{3}\mathrm{He}$ to hydrogen, $[\mathrm{^{3}He/H}] \approx 10^{-5}$, is determined by Big Bang nucleosynthesis. 
I adopt the common assumptions $\frac{\mathit{H}(z)}{(1+\mathit{z})(dv/dr)} \sim 1$ and $\rm{\mathit{T}_{s} \sim \mathit{T}_{\mathrm{gas}}}$.

The power spectrum (PS) of the differential brightness temperature is defined as:

\begin{align}
    \label{ps-equ}
    \rm{\mathit{P}(k) = \langle \ \mathit{\delta T}_{b,^{3}\rm{He}} (k) \mathit{\delta T}_{b,^{3}\rm{He}}(k)^{*} \rangle},
\end{align}
where $\rm{\mathit{\delta T}_{b,^{3}\rm{He}} (k)}$ is the Fourier transform of the differential brightness temperature field, and $\rm{\mathit{\delta T}_{b,^{3}\rm{He}} (k)^{*}}$ is its complex conjugate. 
In the following, I will express the results in terms of the dimensionless power spectrum, defined as:

\begin{align}
    \rm{\Delta_{^{3}He}^{2} = \frac{\mathit{k}^{3}}{2 \pi^{2}} \mathit{P}(k)}.
\end{align}



\begin{figure}
\centering
    \includegraphics[width=100mm]{figures/helium_deltatb_dist.pdf}
    \caption{Volume filling factor of differential brightness temperature of the hyperfine transition of $^{3}\rm{He}^{+}$ at $z\approx4.18$ (solid red curve), 3.28 (dotted green) and 2.90 (dash-dotted blue).}
    \label{deltatb_dist}
\end{figure}


\section{Results}
\label{results}

In this section, I discuss the features and potential observables of 3.5 cm transition line extracted from the helium reionization simulations introduced in AB24.

\subsection{Qualitative Overview}

First, in Figure \ref{deltatb_map}, I present maps of $\delta T_{\mathrm{b},^{3}\mathrm{He}}$ for a slice of the simulation box at three different redshifts: $z \approx 4.18$, $3.28$, and $2.90$. The choice of redshifts
is influenced by the observations of \citealt{Trott2024}. At $z \approx 4.18$, the majority of the volume remains dominated by He\,\textsc{ii}, resulting in relatively high values of $\delta T_{\mathrm{b},^{3}\mathrm{He}}$, typically exceeding $10\,\mu\mathrm{K}$. However, in regions that have been fully ionized to He\,\textsc{iii} by the ionizing radiation emitted by quasars, $\delta T_{\mathrm{b},^{3}\mathrm{He}}$ drops sharply to approximately $10^{-5}\,\mu\mathrm{K}$. As the redshift decreases to $z \approx 3.28$, the regions with low $\delta T_{\mathrm{b},^{3}\mathrm{He}}$ values expand, reflecting the growing percolation of He\,\textsc{iii} regions throughout the volume. This transition signifies the continued progress of helium reionization as more He\,\textsc{ii} is ionized. By $z \approx 2.90$, nearly the entire slice of the simulation box exhibits low $\delta T_{\mathrm{b},^{3}\mathrm{He}}$ values, marking the near-completion of helium reionization. The uniformity of the signal at this stage suggests that most of the helium has transitioned to the fully ionized He\,\textsc{iii} state.

For a more quantitative analysis, Figure~\ref{deltatb_dist} shows the volume filling factor of $\delta T_{\mathrm{b},^{3}\mathrm{He}}$ at the same redshifts as the slice maps in Figure~\ref{deltatb_map}. At all redshifts, the volume filling factor shows a strong double-peaked structure. The peak at higher $\delta T_{\mathrm{b},^{3}\mathrm{He}}$ values corresponds to regions where helium is still singly ionized, while the lower peak is linked to areas where helium has been fully ionized to He\,\textsc{iii}. At $z \approx 4.18$, the fraction is dominated by a strong peak around $1\,\mu\mathrm{K}$, which is over two orders of magnitude higher than the secondary peak at $\delta T_{\mathrm{b},^{3}\mathrm{He}} \sim 10^{-3}\,\mu\mathrm{K}$. At this redshift, there is a third peak towards an even lower value, at $\delta T_{\mathrm{b},^{3}\mathrm{He}} \sim 10^{-4}\,\mu\mathrm{K}$, but with a very low volume filling factor. By $z \approx 3.28$, the volume filling factor at $\delta T_{\mathrm{b},^{3}\mathrm{He}} \lesssim 0.1\,\mu\mathrm{K}$ increases significantly due to ongoing helium reionization, while the contribution from higher emission regions declines. At $z \approx 2.90$, the peak prominence shifts entirely to lower $\delta T_{\mathrm{b},^{3}\mathrm{He}}$ values, with the dominant peak centered around $4 \times 10^{-4}\,\mu\mathrm{K}$, marking the completion of helium reionization.

%In the following sections, I will more focus on the observable quantities related to this 3.5 cm transition line and their trends with redshifts. 


\subsection{Simulated 3.5 cm signal}

I start exploring the features of the $^{3}\mathrm{He}^{+}$ hyperfine transition line by showing the volume-averaged $\delta T_{\rm{b},^{3}\rm{He}}$ (say, $\langle \delta T_{\rm b,\, ^3He} \rangle$) over the entire simulation box 
in Figure \ref{3he_evolution}. Throughout the entire redshift range $\langle \delta T_{\rm b,\, ^3He} \rangle$ remains positive because $T{\rm _S}$ is always higher than the CMB temperature (see Equation \ref{deltatb_formula}). 
The redshift evolution of $\langle \delta T_{\rm b,\, ^3He} \rangle$ closely follows the one of the He~{\sc ii} fraction (see Figure \ref{fig:xheii}), with a nearly constant value until $z\approx4$, when about 15\% of He~{\sc ii} has been ionized. At lower redshift the average signal starts to decline rapidly, reaching $\approx 2.5 \times 10^{-2}$ by $z\approx 2.3$. This drop is linked to the completion of helium reionization.  

To track how fluctuations in the global 3.5 cm signal evolve over time, in the bottom panel of the figure I examine the evolution of the standard deviation of $\delta T_{b,^{3}\rm{He}}$, say $\sigma_{\delta T_{\rm b,\, ^3He}}$. Initially, the fluctuations increase slightly from about 1.4 $\mu$K at $z\approx 5.5$ to around 1.7 $\mu$K by $z\approx 3$. By this time, about 80\% of the He~{\sc ii} in the simulation volume has been fully ionized into He~{\sc iii}. After $z\approx 3$, the fluctuations start to decrease because the reionization process has smoothed out most variations in the abundance of He~{\sc ii} in the IGM. This transition occurs at a redshift to the one at which the temperature of the IGM at mean density begins to saturate, as observed in Figure \ref{fig:temp_evol}. The small fluctuations observed at the lowest redshift are induced by density fluctuations in the IGM. 


\begin{figure}
\centering
    \includegraphics[width=100mm]{figures/He3_signal_evolution.pdf}
    \caption{\textit{Top panel: } Redshift evolution of the volume averaged differential brightness temperature of the hyperfine transition of $^{3}\rm{He}^{+}$. \textit{Bottom:} corresponding standard deviation of this simulated signal.}
    \label{3he_evolution}
\end{figure}

\begin{figure}
\centering
    \includegraphics[width=90mm]{figures/helium_PS.pdf}
    \caption{Spherically averaged differential brightness temperature fluctuations of the 3.5~cm signal at $z\approx4.18$ (solid red curve), 3.28 (dotted green) and 2.90 (dash-dotted blue). Observational upper limits from \citealt{Trott2024} at the same redshifts are shown as circles.}
    \label{ps}
\end{figure}

Similarly to the 21 cm line, the power spectrum of the signal is expected to be the first detectable quantity. Thus, in Figure \ref{ps} I present $\rm{\Delta_{^{3}He}}(\mathit{k})$. All curves increase towards higher $k$ values, indicating stronger fluctuations at smaller spatial scales. During the early stages (at $z\gtrsim 5$), $\rm{\Delta_{^{3}He}}(\mathit{k})$ is mainly dominated by the over-density of gas matter and the inhomogeneous temperatures from the hydrodynamic simulations.
%(although these are not specifically shown in this chapter, however, those are primarily mirroring our ICs, so by definition there is a very slight amount of He~{\sc iii}). 
 As reionization proceeds, the impact of quasars emerges in a scale dependent way. 
From $z \approx 4.18$ to $3.28$, the amplitude of the fluctuations at $\rm{k \gtrsim 0.2 \, \mathit{h} \, Mpc^{-1}}$ (corresponding to spatial scales of $\leq 50 \, \rm{\mathit{h}^{-1} \, Mpc}$) remains largely unchanged, while it drops by $z\approx2.90$. Essentially, the quasars radiation increases the gas temperature in their vicinity, reducing the fluctuations of $\rm{\mathit{\delta T}_{b,^{3}\rm{He}}}$, as well as the amplitude of  $\rm{\Delta_{^{3}He}}(\mathit{k})$. On the larger spatial scales, the effect of the inhomogeneous heating becomes relevant (see also, \citealt{pritchard2007}), increasing the amplitude of $\rm{\Delta_{^{3}He}}(\mathit{k})$ from $z \approx 4.18$ to $3.28$ (when, the $\rm{\mathit{x}_{HeII}}$ drops from $85\%$ to less than $50\%$, see also Figure \ref{fig:xheii}). By $z \approx 2.90$, $\rm{\Delta_{^{3}He}}(\mathit{k})$ decreases further since the majority of the simulation volume is fully ionized, and fluctuations are reduced at all scales.

In the Figure I also include the first observational upper limits on the 3.5~cm brightness temperature fluctuation from \citealt{Trott2024}, which remain consistently about 3-4 orders of magnitude higher than my theoretical predictions. This is primarily attributed to the adopted simple model of foreground emission in \citealt{Trott2024} and to the sensitivity limitations of the telescopes.

\subsection{Cross-correlation of 3.5 cm signal with quasars}

\begin{figure}
\centering
    \includegraphics[width=100mm]{figures/He3_QSO3cm_correlation_Ps.pdf}
    \caption{\textit{Top panel:} 3.5cm - QSO dimensionless cross power spectra at $z\approx4.18$ (solid red curve), 3.28 (dotted green) and 2.90 (dash-dotted blue). \textit{Bottom:}  Corresponding cross-correlation coefficient. The black dotted curve denotes the zero correlation as a reference.}
    \label{he3_qso_crossPS}
\end{figure}

As discussed by \citealt{lidz2009}, cross-correlation between galaxies and 21 cm emission promises to be an excellent probe of the EoR, as it is sensitive to the size and filling factor of H~{\sc ii} regions, and it would alleviate the effect of observational systematics. 
%During most of the reionization process, the 21 cm signal and galaxy distribution are anti-correlated on large scales, but on smaller scales, below the size of the ionized bubbles around galaxies, the two fields become uncorrelated. 
This topic has been extensively investigated in recent years \citep{wiersma2013,vrbanec2016,hutter2018,vrbanec2020,hutter2023,laplante2023,hartman2025}. 
A similar approach could be applied to the 3.5 cm signal, as it could provide additional information on the timing and morphology of helium reionization. 
To explore this, we compute the cross-power spectrum between the differential brightness temperature of the \(^3\mathrm{He}^+\) signal and the spatial distribution of quasars in my simulations. The quasar density field is characterized by the density contrast \(\delta_{\text{QSO}}(\mathbf{x}) = \frac{n_{\text{QSO}}(\mathbf{x})}{\langle n_{\text{QSO}} \rangle} - 1\), where \(n_{\text{QSO}}(\mathbf{x})\) is the local number density of quasars and \(\langle n_{\text{QSO}} \rangle\) is its spatial average. Following the methodology of \citealt{lidz2009}, we calculate the cross-power spectrum as a function of wave number \(k\), which corresponds to different spatial scales. The top panel of Figure~\ref{he3_qso_crossPS} shows the resulting cross-power spectrum, while the bottom panel presents the corresponding cross-correlation coefficient, defined as \(r_{21,\text{gal}}(k) = \frac{P_{21,\text{gal}}(k)}{\sqrt{P_{21}(k) P_{\text{gal}}(k)}}\), where \(P_{21,\text{gal}}(k)\) is the cross-power spectrum, and \(P_{21}(k)\) and \(P_{\text{gal}}(k)\) are the auto-power spectra of the \(^3\mathrm{He}^+\) signal and quasar density field, respectively. 

Early in the helium reionization process, at redshift \( z \approx 4.18 \), we observe that the cross-power spectrum increases from the lowest \( k \) values, gradually gets saturated, peaks around \( k \sim 0.8 \, \rm{h\, cMpc^{-1}} \), and then decreases at higher \( k \) values. The corresponding cross-correlation coefficient is interesting: we see a positive correlation between quasars and the 3.5 cm signal on the largest spatial scales (\( k \lesssim 0.1 \, \rm{h\, cMpc^{-1}} \)), though with significant scatter. At this stage, quasars are still very rare and have just begun ionizing their surroundings. Quasars tend to turn on first in large-scale overdense regions, which contain more matter and initially more neutral hydrogen than underdense regions. As a result, these overdense regions appear brighter in the 3.5 cm emission, leading to a positive cross-correlation on large scales. As ionized bubbles grow, these regions dim in the 3.5 cm signal, while underdense regions, which mostly lack quasars, keep their original emission. This shift causes the correlation to weaken for a short time. As helium reionization continues, by \( z \approx 3.28 \), the amplitude of the cross-power spectrum drops, and the peak moves to larger spatial scales (causing higher amplitude in the lowest \( k \) bins). By this redshift, the 3.5 cm signal and quasar distribution become more anti-correlated, with the correlation coefficient turning negative up to \( k \sim 1 \, \rm{h\, cMpc^{-1}} \), which corresponds to the typical size of He~{\sc iii} bubbles. By \( z \approx 2.9 \), when most of the volume has been reionized, the cross-power spectrum continues to decline at all scales, and the anti-correlation shifts to lower \( k \) values. On small spatial scales (high \( k \)), the cross-correlation coefficient approaches zero, meaning the 3.5 cm signal and quasars become effectively uncorrelated. This illustrates that the 3.5 cm-quasar cross power spectrum provides a relatively direct probe of He~{\sc iii} bubble growth and can be explored to gain more information about the morphology of the helium reionization process.


\section{Discussion and Conclusions}
\label{conclusion}

In this study, I investigated the $^{3}\mathrm{He}^{+}$ hyperfine transition line at 8.67 GHz (3.5 cm) as a novel probe of helium reionization in the IGM, focusing particularly on the redshift range $z < 5$. Using the most recent simulations of helium reionization \citep{basu2024} run by post processing outputs from the hydrodynamic simulation \texttt{TNG300} \citep{volker2018,naiman2018,marinacci2018,pillepich2018,nelson2018} with the radiative transfer code \texttt{CRASH} \citep{ciardi2001,maselli2003,maselli2009,Maselli2005,partl2011}, I examined the spatial and temporal evolution of the 3.5 cm signal and its connection to the ionization state of helium driven by quasars. I also discuss relevant probes related to this signal to constrain the helium reionization. My main findings are as follows -

\begin{itemize}
    \item The spatial distribution of the differential brightness temperature, $\delta T_{\rm b,\, ^3He}$, shows a clear transition from He\,\textsc{ii}-dominated regions at $z \approx 4.18$ to He\,\textsc{iii}-dominated regions by $z \approx 2.90$. The signal intensity drops from values $\gtrsim 1\,\mu$K to $\lesssim 0.1\,\mu$K as reionization progresses.

    \item  The volume-averaged $\delta T_{\rm b,\, ^3He}$ remains relatively constant until $z \sim 4$, after which it declines sharply, mirroring the evolution of the He\,\textsc{ii} fraction. The standard deviation increases slightly during the early stages of reionization and then decreases as the IGM becomes more ionized and uniform.

    \item The 3.5 cm power spectrum, \( \Delta_{\rm 3He}(k) \), increases with \( k \), indicating stronger small-scale fluctuations. Initially, it is driven by gas density and temperature variations. As quasars heat the gas, small spatial scale fluctuations remain largely unchanged, while it drops by \( z \approx 2.9 \). The large-scale fluctuations rises first from $z\approx 4.18$ to 3.28, and decline further by \( z \approx 2.9 \) as the helium reionization process completes.

    \item The simulated power spectra are 3–4 orders of magnitude below the current observational upper limits set by \citealt{Trott2024}. This highlights the challenge of detecting the signal with current instruments and the need for next-generation telescopes like \texttt{SKA}.

    \item At \( z \approx 4.18 \), the 3.5 cm–quasar cross-power spectrum rises, peaks near \( k \sim 0.8\, h\, \mathrm{cMpc}^{-1} \), then declines. A positive large-scale 3.5 cm–quasar correlation (\( k \lesssim 0.1 \)) appears early, as rare quasars ionize overdense, bright regions. As ionized bubbles grow, this correlation weakens. By \( z \approx 3.28 \), the cross power spectrum spectrum drops, shifts to larger scales, and shows anti-correlation up to \( k \sim 1\, h\, \mathrm{cMpc}^{-1} \). At the end of the reionization process, the spectrum declines further and the correlation vanishes on small scales.

\end{itemize}

Overall this study highlights the utility of the $^{3}\mathrm{He}^{+}$ hyperfine transition line as a probe to explore the later stages of cosmic reionization driven by quasars. The significant difference between my theoretical predictions and the current observational upper limits, as we investigated in this chapter, points to the difficulties in detecting this signal. To obtain more reliable insights, future observational campaigns should focus on high signal-to-noise ratios, complementing ongoing efforts to observe the 21-cm signal. Future research will aim to include instrumental noise and foreground modeling in simulations to improve our understanding of observational constraints.  The increased sensitivity of the \texttt{SKA} (especially \texttt{SKA-mid}), along with complementary studies of helium reionization will play a crucial role in advancing our models of the $^3\mathrm{He}^+$ hyperfine signal, improving detection prospects and the understanding of the final stage of cosmic reionization in a more detailed way. 

